Reverberant Audio Source Separation via Sparse and Low-Rank Modeling

The performance of audio source separation from underdetermined convolutive mixture assuming known mixing filters can be significantly improved by using an analysis sparse prior optimized by a reweighting l1 scheme and a wideband datafidelity term, as demonstrated by a recent article. In this letter, we show that the performance can be improved even more significantly by exploiting a low-rank prior on the source spectrograms.We present a new algorithm to estimate the sources based on i) an analysis sparse prior, ii) a reweighting scheme so as to increase the sparsity, iii) a wideband data-fidelity term in a constrained form, and iv) a low-rank constraint on the source spectrograms. Evaluation on reverberant music mixtures shows that the resulting algorithm improves state-of-the-art methods by more than 2 dB of signal-to-distortion ratio.

==> biographies.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/sarberet.jpg}}]{Simon Arberet}
was born in France in 1980. He graduated from \'Ecole Sup\'erieure d'\'Electricit\'e (Sup\'elec), Paris, France in 2003. He received the BA degree in music from University of Paris 8, France, in 2004 and the M.S. degree in computer science from the Pierre and Marie Curie University (Paris 6), France in 2005. He received the Ph.D degree in signal processing from University of Rennes 1, France in 2008. He was with the National Center for Scientific Research (CNRS) from 2005 to 2008 while working towards his Ph.D degree. He worked with the National Institute for Research in Computer and Control Science (INRIA) in 2009. He was scientific researcher at  the 
Signal Processing Laboratory (LTS2), Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL) from 2009 to 2012, and he is now with the Swiss Center for Electronics and Microtechnology (CSEM).
His research interests include statistical signal processing, 
sparse models and algorithms in signal/image processing,  inverse problems and 
 blind audio source separation.
\end{IEEEbiography}





\begin{IEEEbiographynophoto}{Pierre Vandergheynst }
received the M.S. degree in physics and the Ph.D. degree in mathematical physics from the Universit\'e catholique de Louvain, Louvain-la-Neuve, Belgium, in 1995 and 1998, respectively. From 1998 to 2001, he was a Postdoctoral Researcher with the Signal Processing Laboratory, Swiss Federal Institute of Technology (EPFL), Lausanne, Switzerland. He was Assistant Professor at EPFL (2002-2007), where he is now an Associate Professor. 
His research focuses on harmonic analysis, sparse approximations and mathematical data processing in general with applications covering signal, image and high dimensional data processing, sensor networks, computer vision.
He was co-Editor-in-Chief of Signal Processing (2002-2006) and Associate Editor of the IEEE Transactions on Signal Processing (2007-2011), the flagship journal of the signal processing community. He has been on the Technical Committee of various conferences, serves on the steering committee of the SPARS workshop and was co-General Chairman of the EUSIPCO 2008 conference. 
Pierre Vandergheynst is the author or co-author of more than 70 journal papers, one monograph and several book chapters. He has received two IEEE best paper awards.
Professor Vandergheynst is a laureate of the Apple 2007 ARTS award and of the 2009-2010 De Boelpaepe prize of the Royal Academy of Sciences of Belgium.
\end{IEEEbiographynophoto}



\begin{IEEEbiography}[{\includegraphics[width=1.0in,height=1.25in,clip,keepaspectratio]{figures/pic_carrillo.pdf}}]
{Rafael E. Carrillo}
(S'07--M'12) received the B.S. and the M.S. degrees (with honors) in Electronics Engineering from the Pontificia Universidad Javeriana, Bogot\'{a}, Colombia, in 2003 and 2006 respectively and the Ph.D. degree in Electrical Engineering from the University of Delaware, Newark, DE, in 2011. He was a visiting lecturer from 2003 to 2006 at the Pontificia Universidad Javeriana and a Teaching Fellow at the University of Delaware from 2009 to 2011. Currently, he is a postdoctoral researcher at the Institute of Electrical Engineering, Ecole Polytechnique F{\'e}d{\'e}rale de Lausanne, Lausanne, Switzerland.
His research interests include signal and image processing, compressive sensing, inverse problems, and robust, nonlinear and statistical signal processing. Dr. Carrillo was the recipient of the ``Mejor trabajo de grado'' award, given to outstanding master thesis at the Pontificia Universidad Javeriana, in 2006, the University of Delaware Graduate Student Fellowship in 2007 and the Signal Processing and Communications Graduate Faculty Award from the University of Delaware in 2010.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/Thiran-2010-2.jpg}}]{Jean-Philippe Thiran}
(S'91--M'98--SM'03) received the Elect. Eng. and Ph.D. degrees from the Universit\'e catholique de Louvain, Louvain-la-Neuve, Belgium, in 1993 and 1997, respectively. Since 2004 he has been a Professor at the Ecole Polytechnique F\'ed\'erale de Lausanne (EPFL), Lausanne, Switzerland, and director of the Signal Processing Laboratory (LTS5) at EPFL.  Since 2011 he also holds a part time Associate Professor position with the University Hospital Center (CHUV) and University of Lausanne (UNIL). His current scientific interests include image segmentation, prior knowledge integration in image analysis, partial differential equations and variational methods in image analysis and multimodal signal processing, with many applications including remote sensing, medical imaging and human-computer interactions. 
Dr. Thiran was Co-editor-in-Chief of the ``Signal Processing'' international journal from 2001 to 2005. He is currently an Associate Editor of IEEE Transactions on Image Processing. Among many other scientific duties, he was the General Chairman of the 2008 European Signal Processing Conference (EUSIPCO 2008), a tutorial co-chair of the IEEE Int. Conf. on Image Processing in 2011 (ICIP-2011) and will be the technical co-chair of ICIP-2015. He is a Senior Member of the IEEE, member of the IVMSP technical committees of the IEEE Signal Processing Society.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/yvesWiaux.jpg}}]{Yves Wiaux}
 received the M.S. degree in physics and the Ph.D. degree in
  theoretical physics from the Universit\'e catholique de Louvain
  (UCL), Louvain-la-Neuve, Belgium, in 1999 and 2002, respectively.

  He was a Postdoctoral Researcher at the Signal Processing
  Laboratories of the Ecole Polytechnique F\'ed\'erale de Lausanne
  (EPFL), Switzerland, from 2003 to 2008. He was also a Postdoctoral
  Researcher of the Belgian National Science Foundation (F.R.S.-FNRS)
  at the Physics Department of UCL from 2005 to 2009. He is now a
  Senior researcher at the Departments of radiology of the University of
  Geneva and the Lausanne University Hospital, Switzerland,
  with joint affiliation to EPFL. His research lies at the intersection between
  signal processing (inverse problems, sparsity, compressed sensing) and
  applications to biomedical imaging (magnetic resonance) and 
  astronomical imaging (interferometry) and data analysis (cosmic
  microwave background).
\end{IEEEbiography}





==> lowrankProjection.tex <==
\section{Projection onto the set of low-rank matrices\label{sec_lowrankProjection}}

%$f_1(\mathbf{s} ) = \|  \mathbf{s} \stftFrame  \|_{\weightMtx,1}$, 
%$f_2(\mixop(\mathbf{s})) = i_{\mathcal{B}_{\ell_2}^{\epsilon}}( \mixop(\mathbf{s}))$  with 
%$\mathcal{B}_{\ell_2}^{\epsilon} = \{\mathbf{s}  \in \mathbb{R}^{N \times \nbsamples} \ |\ \|\mathbf{s} -  \mathbf{x} \|_2 \leq\epsilon \}$
%$L_2 = \mixop$
%$f_3(\mathbf{s}) = i_{\mathcal{R}^{\rindice}}(\mathbf{s}) $ where $|\cdot|$  is the element-wise modulus operator. 

The best rank-$k$ approximation of a matrix $\mathbf{z}$ with respect to both the Frobenius and spectral norms has an analytic solution 
%in terms of the singular value decomposition (SVD) of $\mathbf{z}$ 
given by the Eckart-Young theorem \cite{eckart1936approximation}. 
Indeed, the projection $\LRProj(\mathbf{z}) = \argmin_{\mathbf{y}}\left\{ \| \mathbf{y} - \mathbf{z} \|_F: \mathbf{y} \in \LRset \right\}$ of a matrix $\mathbf{z}$, onto the (non-convex) set $\LRset = \left\{\mathbf{z} : \rank(\mathbf{z})\leq \rindice \right\}$  of matrices having a rank less or equal than $\rindice$ is given by $\LRProj(\mathbf{z}) = \mathbf{u} \mySigma^{\rindice} \mathbf{v}^*$,
 where $\mathbf{z} = \mathbf{u} \mySigma \mathbf{v}^*$ is the singular value decomposition (SVD) of $\mathbf{z}$ and 
 $\mySigma$ is a diagonal matrix with non-increasing entries $\mySigmaEntry_{ii}$, and
 $\mySigmaEntry^{\rindice}_{ii} :=  \left\{ 
  \begin{array}{l l}
   \mySigmaEntry_{ii}  & \quad \text{if $i\leq \rindice$}\\
    0 & \quad \text{if $i > \rindice$.}
  \end{array} \right.$
 
%  in term of the singular value decomposition (SVD) of the data matrix.
%Let $\LRProj : \complexSet^{m\times n} \rightarrow \complexSet^{m\times n} $  denotes the orthogonal projection onto the set $\LRset$. 
%That is, $\LRProj(\mathbf{z}) = \argmin_{\mathbf{y}}\left\{ \| \mathbf{y} - \mathbf{z} \|_F: \mathbf{y} \in \LRset \right\}$.
%It is well known that $\LRProj(\mathbf{z})$ can be computed efficiently by computing the top $\rindice$ singular values and vectors of $\mathbf{z}$.
%Let $\mathbf{z} = \mathbf{u} \Sigma \mathbf{v}^*$, with $\Sigma$ being a diagonal matrix with non-increasing entries $\Sigma(i,i)$, 
% be the singular decomposition of $\mathbf{z}$, then $\LRProj(\mathbf{z}) = \mathbf{u} \Sigma_{\rindice} \mathbf{v}^*$, where 
%$\Sigma_{\rindice}(i,i) :=  \left\{ 
%  \begin{array}{l l}
%   \Sigma(i,i)  & \quad \text{if $i\leq \rindice$}\\
%    0 & \quad \text{if $i > \rindice$.}
%  \end{array} \right.$

In order to find the projection operator associated with function $f_3(\mathbf{s}) = i_{\mathcal{R}^{\rindice}}(\mathbf{s})$,
Let first define $e^{i \angle \mathbf{z}}: \mathbf{z} \mapsto \mathbf{y}=e^{i \angle \mathbf{z}}$ as the element wise phase such that $y_{nm} = e^{i \arg (z_{nm})}$.
%, and $\arg(\mathbf{z}): \mathbf{z} \mapsto \mathbf{y}=\arg(\mathbf{z})$ as the element wise argument such that $y_{nm} = \arg({z_{nm}})$.
Let us now define the set $\LRMagset$ of complex matrices which element-wise magnitude is a low-rank matrix, i.e. $\LRMagset = \left\{\mathbf{z} : \rank(|\mathbf{z}|)\leq \rindice \right\}$, and the projection $\LRMagProj(\mathbf{z})$ onto $\LRMagset$: $\LRMagProj(\mathbf{z}) :=  \argmin_{\mathbf{y}}\left\{ \| \mathbf{y} - \mathbf{z} \|_F: \mathbf{y} \in \LRMagset \right\}$.
The projection operator associated with function $f_3(\mathbf{s}) = i_{\mathcal{R}^{\rindice}}(\mathbf{s})$ is then 
$\mathcal{P}_{\mathcal{R}^{\rindice}}(\mathbf{s})=\left( \LRMagProj \left(|\stftFrameOp(\mathbf{s}_n)| \right) \right)_{1\leq n \leq N}$.
We will now prove that projection $\LRMagProj(\mathbf{z})$ has a closed form solution which is 
$\LRMagProj(\mathbf{z}) = \LRProj( | \mathbf{z} | ) \circ e^{i \angle \mathbf{z}}$, where $\circ$ is the Hadamard product, i.e. the element wise multiplication.\\
Proof:
For any matrices $\mathbf{z}$ and $\mathbf{y}$, we have 
\begin{align}
\| \mathbf{y} - \mathbf{z} \|_F^2  &= \| \mathbf{y} \|_F^2 + \| \mathbf{z} \|_F^2 - 2 \tr(\mathbf{z}^{\tc} \mathbf{y}) \nonumber \\
&= \| \mathbf{y} \|_F^2 + \| |\mathbf{z}| \|_F^2 - 2 \tr \left( \left( |\mathbf{z}|e^{i \angle \mathbf{z}})^{\tc} (|\mathbf{y}|e^{i \angle \mathbf{y}} \right) \right) \nonumber \\
&= \| \mathbf{y} \|_F^2 + \| |\mathbf{z}| \|_F^2 - 2 \tr \left( |\mathbf{z}|^{\transpose}\left(|\mathbf{y}|e^{i (\angle \mathbf{y}-\angle \mathbf{z})} \right) \right) \nonumber \\
& \geq \| \mathbf{y} \|_F^2 + \| |\mathbf{z}| \|_F^2 - 2 \tr (|\mathbf{z}|^{\transpose} |\mathbf{y}|)  \label{eq:lowerboundFro} \\
& = \| |\mathbf{y}| - |\mathbf{z}| \|_F^2. \nonumber
 \end{align}
 The inequality \eqref{eq:lowerboundFro} is an equality when $\angle \mathbf{y} = \angle \mathbf{z}$.
 Thus, for a given matrix $\mathbf{z}$, the matrix $\mathbf{y}$ with a free phase $\angle \mathbf{y}$ that minimizes $\| \mathbf{y} - \mathbf{z} \|_F$ is then the one that minimizes $ \| |\mathbf{y}| - |\mathbf{z}| \|_F^2$ with $\angle \mathbf{y} = \angle \mathbf{z}$.
 %\eqref{eq:lowerboundFro} is a lower bound on $\| \mathbf{y} - \mathbf{z} \|_F^2 $ which is an equality when $\angle \mathbf{y} = \angle \mathbf{z}$.
%We thus see that the minimization $\argmin_{\mathbf{y}}  \| \mathbf{y} - \mathbf{z} \|_F $ is decoupled between the magnitude $|\mathbf{y}|$ part and the phase part $e^{i \angle \mathbf{y}}$.
As a consequence, $ \argmin_{\mathbf{y}} \left\{ \| \mathbf{y} - \mathbf{z} \|_F: \mathbf{y} \in \LRMagset \right\} = \argmin_{\mathbf{y}} \left\{ \| |\mathbf{y}| - |\mathbf{z}|  \|_F: |\mathbf{y}| \in \LRset, \angle \mathbf{y} = \angle \mathbf{z} \right\}  = \LRProj( | \mathbf{z} | ) \circ e^{i \angle \mathbf{z}}$.


==> optimization.tex <==
\section{Optimization Algorithms\label{sec_optim}}

%\subsection{Constrained vs unconstrained problems}
%
%The Lasso (also called Basis pursuit denoising (BPDN)) problem \eqref{eq_Wideband_Lasso} with $\regterm(\tilde{\mathbf{s}}) = \| \tilde{\mathbf{s}} \|_1$
%has an alternative constrained formulation:
%\begin{align}\label{eq_Wideband_CstBPDN}
%\argmin_{\tilde{\mathbf{s}} \in \mathbb{C}^{N \times \nbcoeff}}\ & 
%%\datafit(\mathbf{x},\mathbf{A},\tilde{\mathbf{s}}) 
%\| \tilde{\mathbf{s}} \|_1 \nonumber \\
%\text{subject to}\ & \|\mathbf{x}-  \mixop( \tilde{\mathbf{s}}   \stftFrame^*)  \|_2 \leq \epsilon,
%\end{align}
%which is equivalent to the unconstrained formulation \eqref{eq_Wideband_Lasso} for some (unknown) value of $\lambda$ and $\epsilon$.
%It follows that determining the proper value of $\lambda$ in \eqref{eq_Wideband_Lasso} is akin to determining the power limit of the noise \cite{chen2001atomic}. 
%However, there is no optimal strategy to fix the regularization parameter $\lambda$ even if the noise level is known, therefore constrained problems, such as \eqref{eq_Wideband_CstBPDN}, offer a stronger fidelity term when the noise power is known, or can be estimated a priori.
%
%Moreover, as stated in \cite{kowalski2010beyond, loris2009performance}, algorithms to optimize \eqref{eq_Wideband_CstBPDN} such as FISTA, have some convergence issue for small values of $\lambda$, which is the case in our problem where the noise is very small or null. 
% Indeed, for small $\lambda$, FISTA requires a larger number of iterations to reach convergence, and secondly, its convergence speed strongly depends on the chosen initialization.  \revision{One can refer to \cite{loris2009performance} for more details on the convergence of this algorithm.}
% So as to let the algorithm converge in practice, it is possible to use a \textit{continuation trick} \cite{loris2009performance,kowalski2010beyond} also known as \textit{warm start}, which consists in running the algorithm multiple times, first with a large value of $\lambda$, and then iteratively decrease the value of $\lambda$ and initialize the algorithm with the result of the previous run. This  \textit{continuation trick} is quite efficient in practice, but requires a significant computational effort specially when $\lambda$ is small (i.e. when the noise is small). 

%\subsection{Reweighted $\ell_1$ vs $\ell_1$ minimization}
%
%The $\ell_1$ minimization problem is equivalent to $\ell_0$ minimization when the \textit{forward} operator $\mixop$ (in Eq. \eqref{eq_convolutive_mixture_model_op}) satisfies certain conditions defined in the context of compressed sensing. 
%The main difference between these two problems, is that  the $\ell_0$ minimization does not depend on the magnitudes of the coefficients, while the 
%$\ell_1$ does.
%One way to mimic the minimization behavior of the $\ell_0$ cost is to replace the $\ell_1$ norm in \eqref{eq_Wideband_CstBPDN} by a weighted $\ell_1$ norm \cite{candes2008enhancing}, 
% which is defined, for a vector or a matrix $\mathbf{z}$ with $\nbentries$ entries $z_i$, as $\sum_{i=1}^{\nbentries} w_i |z_i|$. 
%The idea behind the weighted $\ell_1$ norm, is that large weights will encourage small components while small weights will encourage larger components.
%Moreover, if the non-zero components have very small weights, the weighted norm will be independent of the precise value of the non-zero components.
%\revision{As the original signal and weights are not known in advance, the weights are first initialised to have unit value, i.e. the weighted norm corresponds to the $\ell_1$ norm in that case.
%From the solution of this convex problem, the weights are then re-estimated in a way that penalizes more the small coefficients and less the large coefficients.
%The appropriate weights are then computed via a sequence of weighted $\ell_1$ problems. Each of these weights is essentially the inverse of the value of the solution of the previous problem.}
%This procedure has been observed to be very effective in reducing the number of measurements needed for recovery, and to outperform standard $\ell_1$-minimization in many situations, see e.g. \cite{candes2008enhancing,candes2011compressed}.


The analysis sparse problem which was solved in \cite{arberet2013sparse} was the following constrained problem:
\begin{align}\label{eq_analysisL1Pb}
\argmin_{\mathbf{s} \in \mathbb{R}^{N \times T}}\ & 
\| \mathbf{s} \stftFrame  \|_{\weightMtx,1} \nonumber \\
\text{subject to}\ & \|\mathbf{x}-  \mixop( \mathbf{s}) \|_2 \leq \epsilon,
\end{align}
where $\stftFrame$ is either a base or a redundant frame or dictionary, 
$\weightMtx \in \mathbb{R}_+^{N \times \nbcoeff}$ is a matrix with positive entries $\weightcoeff_{ij}$
which is computed at each iteration of the SSRA algorithm \cite{arberet2013sparse} described in section \ref{sec_SSRA} in order to mimic the behaviour of the $\ell_0$ norm minimization.
$\| \mathbf{z}  \|_{\weightMtx,1} \defeq \sum_{i,j} \weightcoeff_{ij} |z_{ij}|$ is the weighted $\ell_1$ norm and 
$\epsilon$ is a bound on the $\ell_2$ norm of the noise $\mathbf{e}$. 

In this paper we want to constrain the rank of the magnitude source spectrum $|\mathbf{s} \stftFrame |$, where   $|\cdot|$  is the element-wise modulus operator, by introducing the additional low-rank constraint 
$\rank (|\mathbf{s} \stftFrame |) \leq \rindice$ into problem \eqref{eq_analysisL1Pb}, resulting in the following optimisation problem:
\begin{align}\label{eq_reweightedL1Pb}
\argmin_{\mathbf{s} \in \mathbb{R}^{N \times T}}\ & 
%\| \weightMtx \circ (\mathbf{s} \stftFrame)  \|_1 \nonumber \\
\| \mathbf{s} \stftFrame  \|_{\weightMtx,1} \nonumber \\
\text{subject to}\ & \|\mathbf{x}-  \mixop ( \mathbf{s}) \|_2 \leq \epsilon,\nonumber \\
& \rank (|\mathbf{s} \stftFrame |) \leq \rindice,
\end{align}

%\subsection{Analysis vs synthesis problems}
%
%The BPDN (constrained \eqref{eq_Wideband_CstBPDN} or unconstrained \eqref{eq_Wideband_Lasso})  defines the optimization in the sparse representation domain finding the optimal representation vector $\tilde{\mathbf{s}}$ and then recovering
%the true signal through the synthesis relation $\mathbf{s} = \tilde{\mathbf{s}}   \stftFrame^*$. 
%These methods are known as \textit{synthesis} based methods in the literature.
%Synthesis-based problems may also be substituted by \textit{analysis} based problems, where instead of estimating a sparse representation
%of the signal, the methods recover the signal $\mathbf{s} $ itself \cite{elad2007analysis}:
%\begin{align}\label{eq_analysisL1Pb}
%\argmin_{\mathbf{s} \in \mathbb{R}^{N \times T}}\ & 
%%\| \weightMtx \circ (\mathbf{s} \stftFrame)  \|_1 \nonumber \\
%\| \mathbf{s} \stftFrame  \|_{1} \nonumber \\
%\text{subject to}\ & \|\mathbf{x}-  \mixop( \mathbf{s}) \|_2 \leq \epsilon,
%\end{align}
%In the case of orthonormal bases, the two approaches are equivalent. 
%However, when $\stftFrame$ is a redundant frame or an overcomplete dictionary, the two problems are no longer equivalent. 
%The analysis of the geometry of the two problems, studied in \cite{elad2007analysis,nam:inria-00602205}, show that there is a large gap between the two formulations.
%One remark to make is that the analysis problem does not increase the dimensionality of the problem (relative to the signal dimension) 
% when overcomplete dictionaries are used. Empirical studies have shown very promising results for the analysis approach \cite{elad2007analysis}. 
%\cite{candes2011compressed} provides a theoretical analysis of the $\ell_1$ analysis problem coupled with redundant dictionaries in the context of compressed sensing.
%


%\subsection{Source recovery guarantees \label{sec_linkwithCS}}
%
%The literature on Compressed Sensing (CS) and sparse recovery gives some insight about the theoretical guarantees to recover the sources from a mixture by solving problem \eqref{eq_analysisL1Pb}.
%
%The sufficient recovery condition for the analysis problem \eqref{eq_analysisL1Pb} depends \cite{candes2011compressed}  both on the analysis sparsity of the sources ($k = \| \mathbf{s} \stftFrame  \|_{0}$) and on properties of the \textit{forward} operator $\mixop$, more precisely its matrix form $\mathbf{A}$.
%The analysis dictionary $\stftFrame$ is supposed to be a tight frame and can be highly  coherent.
%A sufficient condition for accurate recovery, is that the matrix $\mathbf{A}$ satisfies the so-called D-RIP and that the signal has a sparse representation in $\stftFrame$.
%\revision{The D-RIP \cite{candes2011compressed}  is an extension of the restricted isometry property (RIP) for signals spare in a dictionary, which is a generalisation of a  basis, while the RIP is a property that characterizes matrices which are nearly orthonormal, at least when operating on sparse vectors.}
%We do not have any proof of the validity of the D-RIP for matrix $\mathbf{A}$, but there are some clues about the conditions of its validity.
%
%Indeed, $\mathbf{A}$ is a matrix composed of $M \times N$ Toeplitz blocks, each of them corresponding to the convolution with the filter $a_{mn}$.
%It has been shown \cite{haupt2010toeplitz} that Toeplitz matrices satisfy, with an overwhelming probability, the RIP, for filters of length $\filterLength $ having i.i.d. Gaussian (or zero mean bounded distribution) entries, when the sparsity $k$ of the signal of length $\nbsamples $ is such that $k < c \sqrt{\filterLength/\log(\nbsamples)}$, for a constant $c$. Other results \cite{candes2011compressed} show that a lot of matrices that satisfy the RIP (e.g. matrices with Gaussian, subgaussian, or Bernoulli entries) also satisfy the D-RIP.
%If we assume it is also the case for random Toeplitz matrices, we see that, in the case of a single-channel, single-source ``mixture'' ($M=N=1$), the longer the filters, the larger  the sparsity of the sources can be.
%This discussion suggests that the source estimation, solving problem \eqref{eq_analysisL1Pb}, should be better in reverberant conditions, where the filters are long (large $\filterLength$) and 
%where the coefficients of the filters can be relatively well modeled by an i.i.d. Gaussian distribution or zero mean bounded distribution.
%This trend will be confirmed in the experimental section \ref{sec_perf_reverbtime}.



